Asynchronous Model Predictive Control Under Model Mismatch: Stability and Performance Guarantees

Certainty-equivalence model predictive control (CE-MPC) is widely used for its simplicity and efficiency, but theoretical guarantees under asynchronous feedback remain limited. This paper establishes stability and performance guarantees for asynchronous CE-MPC of input-constrained nonlinear systems. We first derive a nominal stability condition and competitive-ratio bound that explicitly account for inter-execution intervals without prescribing a feedback mechanism. A value-function perturbation analysis for quadratic stage costs then accommodates additive, potentially non-smooth model mismatch without constraint qualification conditions. Combining these results yields stability criteria and competitive-ratio bounds for CE-MPC under general asynchronous feedback, including event/self-triggered and multi-step MPC. The guarantees explicitly relate prediction horizon, inter-execution time, and uncertainty magnitude, quantifying performance degradation relative to an ideal infinite-horizon controller. These results clarify tradeoffs between feedback frequency, model accuracy, and horizon length, guiding asynchronous MPC design using approximate or learned models.

==> 1-major_content/8-acknowledgement.tex <==
\section*{Acknowledgment}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/a1.png}}]{First A. Author} (Fellow, IEEE) and all authors may include 
	biographies. Biographies are
	often not included in conference-related papers.
	This author is an IEEE Fellow. The first paragraph
	may contain a place and/or date of birth (list
	place, then date). Next, the author’s educational
	background is listed. The degrees should be listed
	with type of degree in what field, which institution,
	city, state, and country, and year the degree was
	earned. The author’s major field of study should
	be lower-cased.
	
	The second paragraph uses the pronoun of the person (he or she) and
	not the author’s last name. It lists military and work experience, including
	summer and fellowship jobs. Job titles are capitalized. The current job must
	have a location; previous positions may be listed without one. Information
	concerning previous publications may be included. Try not to list more than
	three books or published articles. The format for listing publishers of a book
	within the biography is: title of book (publisher name, year) similar to a
	reference. Current and previous research interests end the paragraph.
	
	The third paragraph begins with the author’s title and last name (e.g.,
	Dr. Smith, Prof. Jones, Mr. Kajor, Ms. Hunter). List any memberships in
	professional societies other than the IEEE. Finally, list any awards and work
	for IEEE committees and publications. If a photograph is provided, it should
	be of good quality, and professional-looking.
\end{IEEEbiography}

\begin{IEEEbiographynophoto}{Second B. Author,} photograph and biography not available at the
	time of publication.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Third C. Author Jr.} (Member, IEEE), photograph and biography not available at the
	time of publication.
\end{IEEEbiographynophoto}

==> 1-major_content/9-biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/changrui_ieee.jpg}}]{Changrui Liu} received the BSc degree (cum laude) from Harbin Institute of Technology (HIT) in Harbin, China, he graduated from Honors School, HIT and was awarded Best 10 Graduate, 2019. He then received the MSc degree from TU Delft, Aerospace Engineering. He is currently pursuing the PhD degree at the Delft Center for Systems and Control, TU Delft. His research interests are performance guarantees in machine learning and optimization.
\end{IEEEbiography}
\vspace*{-1cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/shengling_shi.jpg}}]{Shengling Shi} is an assistant professor at Delft Center for Systems and Control, TU Delft, and he was a postdoctoral associate at the Massachusetts Institute of Technology, USA. He was also a postdoc at the Delft Center for Systems and Control, TU Delft, the Netherlands. He received the Ph.D. degree from the Eindhoven University of Technology in 2021. His research interests include system identification, model predictive control, and their applications.
\end{IEEEbiography}
\vspace*{-1cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bds_2018.jpg}}]{Bart De Schutter} (IEEE member since 2008, senior member since 2010, and fellow since 2019) is a full professor and head of 
department at the Delft Center for Systems and Control of Delft 
University of Technology in Delft, The Netherlands. He is also an IFAC fellow.

Bart De Schutter is a senior editor of the IEEE Transactions on 
Intelligent Transportation Systems and was an associate editor of IEEE Transactions on Automatic Control.  His current research interests 
include integrated learning- and optimization-based control, multi-level and multi-agent control, 
and control of hybrid systems.
\end{IEEEbiography}

==> 1.3-problem/1.3.1-problem_material.tex <==
It is required that $\ell^\star$ is a \textit{relaxed} control Lyapunov function (rCLF) for the nominal model $f$, i.e., there exists $\lyacf \in \bR_+$ such that
\begin{equation}
    \label{eq:sec3-rclf_decay}
    \min_{u \in \cU}\{\ell^\star(f(x,u)) + \cost(x, u)\} \leq (1 + \lyacf)\ell^\star(x).
\end{equation}
Note that \eqref{eq:sec3-rclf_decay} can always be satisfied since $\lyacf$ is allowed to be $+\infty$. The considered CE-MPC adopts $\ell^\star$ as its terminal cost, which is equivalent to MPC formulations without a terminal cost~\cite{liu2026certainty}, a popular approach in both theory and practice~\cite[Chapter 6]{grune2017nonlinear}. 

Denote the solution to $\probmpc{f}$ by $\{u^\star_k(x;f)\}^{N-1}_{k=0}$ and $\{\xi^\star_k(x;f)\}^{N}_{k=0}$, and the optimal value by $V_{N}(x; f)$. From the perspective of parametric programming, $u^\star_0(x;f)$ and $V_{N}(x; f)$ implicitly defines an MPC policy $\pi_{N,f}: \cX \to \cU$ as $\pi_{N,f}(x) = u^\star_0(x;f)$ and a \textit{continuous} MPC value function $V_{N,f}: \cX \to \bR_+$ as $V_{N,f}(x) = V_{N}(x; f)$~\cite{rawlings2017model}. When MPC is formulated using the true model functions $\{f^\ast_k\}^{t+N-1}_{k=t}$, one can analogously define $\probmpc{\{f^\ast_k\}^{t+N-1}_{k=t}}$; its solution, policy, and value function are denoted in the same manner as those of $\probmpc{f}$ by substituting $f$ with $\{f^\ast_k\}^{t+N-1}_{k=t}$. The closed-loop system under the CE-MPC policy is given by
\begin{equation}
    \label{eq:sec3-closed_loop}
    \xcl{t+1}^\ast = \tsys{t}\big(\xcl{t}^\ast, \pi_{N,f}(\xcl{t}^\ast)\big),
\end{equation}
where $\xcl{t}^\ast$ denotes the closed-loop state at time step $t$ under $\pi_{N,f}$. Staring from $\xcl{0}^\ast = x$, the infinite-horizon performance of the CE-MPC controller is given by
\begin{equation}
    \label{eq:sec3-performance}
    J_{\infty}(x;\pi_{N,f}) = \sum^\infty_{t=0}\ell\big(\xcl{t}^\ast, \pi_{N,f}(\xcl{t}^\ast)\big).
\end{equation}
The objective is to (i) investigate the conditions under which $\pi_{N,f}$ stabilizes the true system at the origin asymptotically (i.e., $\lim_{t\to+\infty}\xcl{t}^\ast = \bzero$) and (ii) quantify the suboptimality of $J_{\infty}(x;\pi_{N,f})$ compared to $V_{\infty}(x;\tsysc)$.

==> 1.5-cases/1.5.1-cruise.tex <==
\subsection{Adaptive Cruise Control}






==> 1.5-cases/1.5.2-grid.tex <==
\subsection{Switched Nonlinear Systems}


==> unused.tex <==
%\footnote{Formally, a family of functions $\{f_i: \bR^n \to \bR^n\}_{i\in\mathcal{I}}$ is \emph{uniform-Lipschitz} if there exists a shared constant $L \ge 0$ such that $\|f_i(x) - f_i(y)\| \le L \|x - y\|$ for all $i \in \mathcal{I}$ and all $x,y \in \bR^n$. Equivalently, this means the supremum of their individual Lipschitz constants $L_i$ is bounded: $\sup_i L_i \le L < \infty$.}

